PhyAug: Physics-Directed Data Augmentation for Deep Sensing Model Transfer in Cyber-Physical Systems

Run-time domain shifts from training-phase domains are common in sensing systems designed with deep learning. The shifts can be caused by sensor characteristic variations and/or discrepancies between the design-phase model and the actual model of the sensed physical process. To address these issues, existing transfer learning techniques require substantial target-domain data and thus incur high post-deployment overhead. This paper proposes to exploit the first principle governing the domain shift to reduce the demand on target-domain data. Specifically, our proposed approach called PhyAug uses the first principle fitted with few labeled or unlabeled source/target-domain data pairs to transform the existing source-domain training data into augmented data for updating the deep neural networks. In two case studies of keyword spotting and DeepSpeech2-based automatic speech recognition, with 5-second unlabeled data collected from the target microphones, PhyAug recovers the recognition accuracy losses due to microphone characteristic variations by 37% to 72%. In a case study of seismic source localization with TDoA fngerprints, by exploiting the frst principle of signal propagation in uneven media, PhyAug only requires 3% to 8% of labeled TDoA measurements required by the vanilla fingerprinting approach in achieving the same localization accuracy.

==> Makefile <==
all:
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

dvi:
	#if [ ! -f dvimode ] ; \
	#then \
	#	echo "Entering dvimode" ; \
	#	echo "" > dvimode ; \
	#	sed -i '/\RequirePackage\[prologue\]{xcolor}/c\\\RequirePackage{xcolor}' acmart.cls; \
	#fi;
	#latex -src-specials -halt-on-error main
	pdflatex -synctex=1 -src-specials -interaction=nonstopmode main

bib:
	bibtex main

pdf:
	#if [ -f dvimode ] ; \
	#then \
	#	echo "Exiting dvimode" ; \
	#	rm -f dvimode ; \
	#	sed -i '/\RequirePackage{xcolor}/c\\\RequirePackage\[prologue\]{xcolor}' acmart.cls; \
	#fi;
	#latex main
	#dvips main.dvi
	#ps2pdf main.ps
	pdflatex main

drop:
	unison dropbox ~/research/ai-physics/IPSN-cameraready ~/Dropbox/PhyModnAI/PhyAug_IPSN_submission


==> Makefile_ <==
all:
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

dvi:
	#if [ ! -f dvimode ] ; \
	#then \
	#	echo "Entering dvimode" ; \
	#	echo "" > dvimode ; \
	#	sed -i '/\RequirePackage\[prologue\]{xcolor}/c\\\RequirePackage{xcolor}' acmart.cls; \
	#fi;
	latex -src-specials -halt-on-error main
	pdflatex -synctex=1 -src-specials -interaction=nonstopmode main

bib:
	bibtex main

pdf:
	#if [ -f dvimode ] ; \
	#then \
	#	echo "Exiting dvimode" ; \
	#	rm -f dvimode ; \
	#	sed -i '/\RequirePackage{xcolor}/c\\\RequirePackage\[prologue\]{xcolor}' acmart.cls; \
	#fi;
	#latex main
	#dvips main.dvi
	#ps2pdf main.ps
	pdflatex main

drop:
	unison dropbox ~/research/ai-physics/IPSN-cameraready ~/Dropbox/PhyModnAI/PhyAug_IPSN_submission


==> eps/atr_transfer_func_diff_length.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2520.00,2016.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,384){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(444,636){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(444,888){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(444,1140){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(444,1392){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(444,1644){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(444,1896){\makebox(0,0)[r]{\strut{}$1.2$}}%
      \put(516,264){\makebox(0,0){\strut{}0}}%
      \put(963,264){\makebox(0,0){\strut{}2000}}%
      \put(1410,264){\makebox(0,0){\strut{}4000}}%
      \put(1856,264){\makebox(0,0){\strut{}6000}}%
      \put(2303,264){\makebox(0,0){\strut{}8000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1140){\rotatebox{-270}{\makebox(0,0){\strut{}normalized magnitude}}}%
      \put(1409,84){\makebox(0,0){\strut{}Frequency}}%
      \csname LTb\endcsname%%
      \put(953,1773){\makebox(0,0)[r]{\strut{}5s}}%
      \csname LTb\endcsname%%
      \put(953,1653){\makebox(0,0)[r]{\strut{}30s}}%
      \csname LTb\endcsname%%
      \put(1736,1773){\makebox(0,0)[r]{\strut{}120}}%
      \csname LTb\endcsname%%
      \put(1736,1653){\makebox(0,0)[r]{\strut{}240s}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{../eps/atr_transfer_func_diff_length}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> eps/de-svm-mlp-execution-time-logscale.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2520.00,1764.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,384){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(444,594){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(444,804){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(444,1014){\makebox(0,0)[r]{\strut{}$10^2$}}%
      \put(444,1224){\makebox(0,0)[r]{\strut{}$10^3$}}%
      \put(444,1434){\makebox(0,0)[r]{\strut{}$10^4$}}%
      \put(444,1644){\makebox(0,0)[r]{\strut{}$10^5$}}%
      \put(516,264){\makebox(0,0){\strut{}$4^2$}}%
      \put(968,264){\makebox(0,0){\strut{}$10^2$}}%
      \put(1535,264){\makebox(0,0){\strut{}$10^3$}}%
      \put(2103,264){\makebox(0,0){\strut{}$10^4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1014){\rotatebox{-270}{\makebox(0,0){\strut{}Execution time (ms)}}}%
      \put(1409,84){\makebox(0,0){\strut{}The number of grids $N$}}%
      \put(1140,1144){\makebox(0,0)[r]{\strut{}DE}}%
      \put(1140,1024){\makebox(0,0)[r]{\strut{}SVM}}%
      \put(1140,904){\makebox(0,0)[r]{\strut{}MLP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{../eps/de-svm-mlp-execution-time-logscale}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> svm-mlp-accuracy.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,504){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(444,946){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(444,1387){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(444,1829){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(444,2270){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(444,2712){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(444,3153){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(444,3595){\makebox(0,0)[r]{\strut{}$70$}}%
      \put(444,4036){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(444,4478){\makebox(0,0)[r]{\strut{}$90$}}%
      \put(444,4919){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(516,384){\makebox(0,0){\strut{}500}}%
      \put(2512,384){\makebox(0,0){\strut{}5000}}%
      \put(4730,384){\makebox(0,0){\strut{}10000}}%
      \put(6948,384){\makebox(0,0){\strut{}15000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,2711){\rotatebox{-270}{\makebox(0,0){\strut{}model accuracy (%)}}}%
      \put(3732,204){\makebox(0,0){\strut{}Number of training data}}%
      \put(3237,123){\makebox(0,0)[r]{\strut{}svm}}%
      \put(3948,123){\makebox(0,0)[r]{\strut{}MLP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{svm-mlp-accuracy}}%
    \gplfronttext
  \end{picture}%
\endgroup

